Reconstructing Actions To Explain Deep Reinforcement Learning

Feature attribution has been a foundational building block for explaining the input feature importance in supervised learning with Deep Neural Network (DNNs), but face new challenges when applied to deep Reinforcement Learning (RL).We propose a new approach to explaining deep RL actions by defining a class of \emph{action reconstruction} functions that mimic the behavior of a network in deep RL. This approach allows us to answer more complex explainability questions than direct application of DNN attribution methods, which we adapt to \emph{behavior-level attributions} in building our action reconstructions. It also allows us to define \emph{agreement}, a metric for quantitatively evaluating the explainability of our methods. Our experiments on a variety of Atari games suggest that perturbation-based attribution methods are significantly more suitable in reconstructing actions to explain the deep RL agent than alternative attribution methods, and show greater \emph{agreement} than existing explainability work utilizing attention. We further show that action reconstruction allows us to demonstrate how a deep agent learns to play Pac-Man game.

==> 03_Method.tex <==

%\section{Evaluation Beyond Visualization}
\section{Attribution Policy}
In deep RL, we consider a policy as a mapping from the state space to the action space $\pi:\mathcal{S}\rightarrow\mathcal{A}$, which guides the agent to make a decision. \todo{Motivation} On the other hand, we are also interested in defining an attribution policy $\Pi$ that guides us to interpret an attribution map into an action. A similar concept, action reconstruction, has been discussed by~\citet{Annasamy2019TowardsBI} where the authors manage to use key-values in the proposed attention layer~\cite{Bahdanau2015NeuralMT} to reconstruct an action. 

\subsection{What Makes a Good $\Pi$?}

\begin{itemize}
	\item \textbf{\todo{Placeholder}.} (Discuss the agent-environment interaction.)
	\item \textbf{Objectivity.} Visualization is the most common approach to interpret an attribution map. However, an visualization itself does not reconstruct the action. Based on an user's bias and domain knowledge, a $\Pi$ can be subjective. For example, the authors argue that \textit{The agent is positioning its own paddle, which allows it to return the ball at a specific angle}~\cite{Greydanus2018VisualizingAU}. However, different users can develop distinctive and sometimes contradictory descriptions for the same attribution map. \citet{Atrey2020ExploratoryNE} points out most of the existing work in explaining DQN agent lacks sufficient quantitative metrics to justify the provided attribution is faithful to the model, and most of their descriptions disagree with the agent's behavior if examined with counterfactual analysis. 
\end{itemize}
\subsection{Proposed Attribution Policy: $\lambda$-LRA}

\subsection{Evaluation: $\lambda$-Alignment}

Visual comparisons between attribution maps can be less objective and sometimes enven misleading. However, as pointed out by \citet{Atrey2020ExploratoryNE}, most of the existing work in explaining DQN agent lacks sufficient quantitative metrics to justify the provided attribution is a good explanation. Among multiple criteria that defines a good attribution, we are interested in whether the attribution scores are proportional to the actual importance of features that drive the agent to make a certain action. Given the ground-truth of the feature importance is unknown, several methods approximates the answer to the question above by measuring if the attribution score is proportional to the change of QoI when the corresponding feature is ablated~\cite{ancona2018towards, NIPS2018_8160, Yeh2019OnT, Wang_2020_CVPR, Bhatt2020EvaluatingAA}. These metrics are designed mainly for classification tasks where we point out two limitations in benchmarking attributions for deep RL models with them:
\begin{itemize}
	\item \textbf{Perturbation as Evaluation.} Most of the metrics are designed to evaluate gradient-based attributions by perturbing the input. As a result, perturbation-based methods are usually treated as the evaluation tool instead of the target to be evaluated. For example, \textit{sensitivity}-$N$~\cite{ancona2018towards} and \textit{faithfulness}~\cite{Bhatt2020EvaluatingAA} are defined by perturbing a subset of input features. As a result of which, OC-1 is by definition the best method under \textit{sensitivity}-$1$. 
	      % \item \textbf{Semantically Meaningful Evaluation.} When evaluating image input, existing metrics tend to do counterfactual analysis by perturbing one pixel or any subset of pixels sampled from the input. However, in RL tasks, a semantically meaningful feature can sometimes, e.g. the food in Pac-Man, consist of a subset of pixel-level features at some particular locations. \citet{Atrey2020ExploratoryNE} discovers the same issue as well and proposes \textit{semantics-preserving} and \textit{fat-hand} perturbations.
	\item \textbf{Action Reconstruction.} An ideal explanation should easily let the user understand why the agent takes a specific action. In the other word, an explanation should be able to let humans to reconstruct the action if some well-defined rules are correctly followed. One frequently used method to reconstruct the action from the input attribution is via users' subjective descriptions. For example, the authors argue that \textit{The agent is positioning its own paddle, which allows it to return the ball at a specific angle}~\cite{Greydanus2018VisualizingAU}. However, different users can develop distinctive and sometimes contradictory descriptions for the same attribution map. Existing metrics do not examine the attribution under the same way of reconstructing the action of interest from the input attribution.
	      % \item \textbf{Input Correlation.} One major difference between RL tasks and the classification is that the inputs for RL model are correlated along the temporal dimension and each action the agent takes influences the input at next timestep for DQN, whereas in the classification task we assume each input is drawn independently from a given distribution.
\end{itemize}
\carlee{I don't quite see how these limitations are unique to RL}

Our method is largely motivated by the \textit{agreement} metric introduced by \citet{Annasamy2019TowardsBI} that firstly builds a rule that reconstruct an action from the key-value in the proposed attention layer~\cite{Bahdanau2015NeuralMT} and compares if the reconstructed action agrees the actual action the agent takes when choosing action QoI with the optimal action at each step. We consider to extend \textit{agreement} to DQNs without attention layers. Firstly we develop a reconstruction rule that maps the input attribution map into an action, which is used to compare with the actual action the agent takes. An ideal input attribution map should optimize the alignment between reconstructed actions and the actions it aims to attribute. We then evaluate each post-hoc attribution map under the same reconstruction function and provide the winner. We first introduce the proposed reconstruction rule $\lambda$-Locally Reconstructed Action with Def.~\ref{def: Optimal Individual Action} and \ref{def: Locally Reconstructed Action}.

\begin{definition}[Optimal Individual Action (OIA)]
	\label{def: Optimal Individual Action}
	Given a Q-network $Q(\avec, \svec) = f(\svec)$, an input feature $s_i$ and an input attribution $g(\svec, \phi_{a})$ that takes an action QoI $\phi_{a}$, the optimal individual action for $s_{i}$ is defined as $ a^\dagger_{i} = \arg\max_{a \in \mathcal{A}} g(\svec, \phi_{a})_i $ where $g(\svec, \phi_{a})_i = z_i$. We denote the one-hot encoding of $a^\dagger_i$ as $\mathbf{a}^\dagger_i$.
\end{definition}

\begin{definition}[$\lambda$-Locally Reconstructed Action ($\lambda$-LRA)]
	\label{def: Locally Reconstructed Action}
	Given a Q-network $Q(\avec, \svec) = f(\svec)$, for an agent whose location in the environment can be determined by a vector $\mathbf{p}$, the optimal individual action $\mathbf{a}^\dagger_i$ for each feature located at $\mathbf{q}_{i}$ under an input attribution $g$, the $\lambda$-Locally Reconstructed Action $\hat{a}_\lambda$ is defined as 
	\begin{align}
		\hat{a}_\lambda = \arg\max_c (\sum_{i \in \mathcal{I}_\lambda}\mathbf{a}^\dagger_i)_c 
	\end{align} where $\mathcal{I}_\lambda$ denote a set of features such that $r(\mathbf{p}, \mathbf{q}_{i}) \leq \lambda, \forall i \in \mathcal{I}_\lambda$ and $r(\cdot, \cdot)$ is an user-defined mapping that measures the distance between a feature and the agent.
\end{definition}

\noindent\textbf{Explanation of OIA.} Each input feature may not be important exclusively for one particular action. Focusing only on the optimal action the agent takes manages to reveal a piece of the full explanation, \textit{how important of this feature is to the optimal action?}, but overlooks an important follow-up, \textit{what action is this feature most important for?}. Therefore, instead of only focusing on the optimal action, we examine all possible action $a \in \mathcal{A}$ and compute the attribution score of an input feature towards $a$. The action towards which a feature receives the highest attribution score is considered to be the action towards which this feature attributes most significantly. \carlee{calling this ``optimal'' may be confusing (it sounds like you are finding the optimal action), maybe ``Most Significant'' instead?}

\noindent\textbf{Restricting the Range.} \carlee{I think this should be introduced earlier, but I am not sure how to yet...} $\lambda$-LRA considers the OIAs of features only within a neighborhood (parameterized by $\lambda$) of the agent valid to the action reconstruction given the fact that future rewards are discounted by $\gamma$ in the training and the agent's each action has limited influence to the environment, e.g. the agent in Pac-Man can only move to its neighboring grid at each timestep. A choice of the distance function $r$ should also reflect rules in the environment; for example, $\ell_1$ distance is a considered as reasonable for Pac-Man since a valid move of the agent is either horizontal or vertical. In the experiment section we will sweep over a broad range of $\lambda$.

\noindent\textbf{Reconstruction Consistency.} We then use the majority of the OIAs from features within a distance of $\lambda$ to reconstruct the action as an input attribution is supposed to be interpreted as. This process is invariant to the method of input attribution. \carlee{emphasize this earlier}

With Def.~\ref{def: Locally Reconstructed Action}, we formally introduce $\lambda$-Alignment as a metric to evaluate an input attribution for DQNs and we end this section with Prop.\ref{prop: better method}.
\begin{definition}[$\lambda$-Alignment]
	\label{Alignment}
	Given a Q-network $Q(\avec, \svec)=f(\svec)$, the $\lambda$-LRA $\hat{a}_\lambda$ from an input attribution $g$  and an action of interest $a$, we define $\lambda$-Alignment $L_\lambda(g, a)$ for an input attribution $g$ as 
	\begin{align}
		L_\lambda(g, a) = \mathbb{E}_{\svec \sim \mathcal{S}} \mathbb{I}[a = \hat{a}_\lambda] 
	\end{align} where $\mathbb{I}$ is an indicator function.
\end{definition}

\begin{proposition}
	\label{prop: better method}
	Given two input attribution methods $g_1$ and $g_2$ with Action QoI,  $g_1$ is $\lambda-$locally more aligned with DQN's decision than $g_2$ if $L_\lambda(g_1, a^*) > L_\lambda(g_2, a^*)$ where $a^* = \arg\max_aQ(a, \svec)$.
\end{proposition}


\section{Attribution Over Time}
\label{sec: method}
In this section, we reuse the notation of $t$ for states $\svec_t$ and actions $a_t$ to distinguish the variables from the current states and those from other timesteps. In the previous section we develop an evaluation tool for the existing attribution methods which locate important features in the input state for a given QoI. In this section, we discuss one weakness of existing methods and propose a new way of attributing input features to understand DQN. 

One major difference between classifications that attribution methods are originally designed for and deep RL is that the inputs of the deep RL are correlated over time due to the fact that the state an agent receives at each timestep is dependent on the last action it took, whereas in classifications, e.g. images, we assume each input is drawn from a given distribution independently. Some features may not directly benefit the agent at the current moment but will bring advantages in the future for the agent (see Example \todo{Example} for an instance). In other words, existing methods only manage to reveal how important features distribute over the spatial dimensions but fail to show how the feature importance distributes over the temporal dimension. Consider the target Q-value in Def.\todo{def} that we want to model with a DQN, let $F(\tau) = \gamma^{\tau-t}R(\tau, a_\tau)$. When choosing the action QoI for the input attribution, we expect that there is an decomposition of the attribution score $z_i$ for each input feature $s_{t, i}$ such that $z_i = \sum^T_\tau z_{\tau, i}$ where each $z_{\tau, i}$ corresponds to the contribution of the feature towards $F(\tau)$, which is defined formally with Def.~\ref{def: TAD}.  
\begin{definition}[Temporal Attribution Decomposition]
	\label{def: TAD}
	Given a Q-network $Q(\avec_t, \svec_t)=f(\svec_t)$, for any QoI that can be decomposed into $\phi(Q(\avec_t, \svec_t)) = \sum^T_{\tau=t} F(\tau)$, a Temporal Attribution Decomposition is an vector $\zvec_{t:T, i} = [z_{t, i}, z_{t+1, i}, ..., z_{T, i}]^\top$ where $z_{\tau, i}$ is the contribution of feature $s_i$ towards $F(\tau)$ and $T$ is the total number of timestes that the agent experiences in the environment before the termination condition is met.
\end{definition}

\begin{definition}[Completeness]
	Given a Q-network $Q(\avec_t, \svec_t)=f(\svec_t)$ and an input attribution $\zvec = g(\svec_t, \phi)$, if $\zvec_{t:T, i}$ is a Temporal Attribution Decomposition of $z_i$ for the feature $s_{t, i}$, then $z_i = \sum^T_{\tau=t} z_{\tau, i}$.
\end{definition}
	
\begin{remark}
	Specifically, in the image or tabular data classification, the network is trained only to predict the label of the current input and the network's prediction will not influence either the next input or the network's decision of the next input. Therefore, for non-RL classification tasks, we treat $z_{\tau, i} = 0, \forall \tau > t$. 	
\end{remark}																																
	
\noindent\textbf{Counterfactual Analysis Over Time.} We use OC-1 as $g(\svec, \phi)$ to calculate the total attribution score $\zvec$ and its decomposition over timesteps instead of gradient-based methods because DQN output is not differentiable through the time, e.g. $\partial \phi_a(f(\svec_{t+1})) / \partial \svec_t = \mathbf{0}$. For each input feature $s_{t, i}$, we create a counterfactual input state $\svec'_{t}$ by perturbing $s_{t, i}$ with a baseline value $b$. 
	
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}
		\begin{scope}[every node/.style={thick,draw, minimum size=0.6cm]}]
				\node (A) at (0.5,0) {$\svec'_t$};
				\node (B) at (0.5,1.7) {$\svec_t$};
				\node (C) at (3,0) {$\svec'_{t+1}$};
				\node (D) at (3,1.7) {$\svec_{t+1}$};
				\node (E) at (1.5,3) {$Q_t$};
				\node (F) at (1.5,-1.3) {$Q'_t$} ;
				\node (G) at (4,3) {$Q_{t+1}$};
				\node (H) at (4,-1.3) {$Q'_{t+1}$} ;
				\node (I) at (5.5,0) {$\svec'_{t+2}$};
				\node (J) at (5.5,1.7) {$\svec_{t+2}$};	
				\node (K) at (6.5,3) {$Q_{t+2}$};
				\node (L) at (6.5,-1.3) {$Q'_{t+2}$} ;					
			\end{scope}
																																																																																																																																																																																																																																																																																										
			\begin{scope}[>={Stealth[black]},
					every node/.style={fill=white,circle},
				every edge/.style={draw=black,thick}]
				\path [->] (B) edge[draw=red] (A);
				\path [->] (A) edge (F);
				\path [->] (B) edge (E);
				\path [->] (B) edge node {$a_t$} (D);
				\path [->] (A) edge node {$a_t$} (C);
				\path [->] (C) edge node {$a'_{t+1}$} (I);
				\path [->] (D) edge node {$a_{t+1}$} (J);
				\path [->] (D) edge (G);
				\path [->] (C) edge (H);
				\path [->] (J) edge (K);
				\path [->] (I) edge (L);
																																																																																																																																																																																	
			\end{scope}
		\end{tikzpicture}
		\caption{placeholder}
		\label{fig: Towards Interpretable Reinforcement Learning}
	\end{figure}
	% \subsection{Motivation}
	% % Definition:
																																																																																																																																																	
	% \subsection{Comment -- Perturbation-based Saliency}
	% The optimal action: $ \hat{a} = \operatorname{argmax}_{a^{\prime} \in A} Q\left(s, a^{\prime}\right)$
																																																																																																																																																	
	% Denote the state feature map as $s\in R^{m\times n}$, the action space as $\mathcal{A}$ where $|\mathcal{A}| = c$ and a Q-value function $Q(s,a)$. Following a greedy policy, denote the action selected by the agent at state $s$ as $\hat{a}$, i.e. $\hat{a} = \arg\max_a Q(s,a_i), i \in [0, c]$. We are interested in identifying which object $o$ of one feature at  state $s$ is important to the agent in taking action $\hat{a}$. For each object $o$, first perturb $s$ to get $s\prime$. For instance, in Pacman, we can perturb food feature by removing one food dot. Then we use softmax to normalize the Q values.
	% \begin{align}
	% 	P(s_t,a_i) = \frac{exp(\gamma Q_t(s, a_i)+(1-\gamma)Q_{t+1}(s_{t+1},a_i))}{\sum_i exp(Q_t(s_t, a_i))} 
	% \end{align}
	% and compute the difference $\Delta p_{a_{i}} = P(s_t, a_i) - P(s_t\prime, a_i)$ between perturbed state and original one. The action that object $o_j$ of feature $f$ represents is: $a_{o_{j}} = \arg\max_a \Delta p_{a_{i}}$. We interpret the $a_{o_{j}}$ as the action that object $o_j$ supports the agent under current environment.
																																																																																																																																																	
	% For each state $s$, we can get one feature's attribution map $z$ by iterating all of the objects within this feature and compute $a_{o_{j}}$ for each object. 
																																																																																																																																																	
																																																																																																																																																	
	% % 
	% Knowing which part of the input pose important influences, spatially, is interesting and could help us to have an intuitive understanding of agents' strategies. In order to use saliency map visualizing important area of the input, the most intuitive way to perform is to apply perturbation to the input and see how this influence the decision agents make. 
																																																																																																																																																	
	% \subsection{Comment -- Definition of Perception Range:}
	% In food matrix $M_{food}$, 
																																																																																																																																																	
	% for position $p_{food}$, 
																																																																																																																																																	
	% the position of MsPacman $p_{pacman}$, 
																																																																																																																																																	
	% the L1 distance: $d_{L_1}(p_{food}, p_{pacman})$,
																																																																																																																																																	
	% Food in a certain perception range $V(d)$ is:
	% a set of positions $P$, where $p_i \in S_P$ has distance 
	% $$d_{L_1}(p_i, p_{pacman}) \leq d$$
																																																																																																																																																	
	% intuitively is the point set where food lies within a L1 distance radius $d$.
																																																																																																																																																	
	% \subsection{Comment -- Definition of Coverage (Alignment Ratio):}
																																																																																																																																																	
	% Assume pacman is located at $(u, v)$ $p_{pacman}$ in the state feature map. Therefore, we build a subset of object indices $S_r$ such that $\forall (i,j)\in S_r$ we have $||s_{i, j} - s_{u, v}||_p \leq r$.  Denote the appearance frequency of action $a_{i}$ in attribution map $z$ as $f_{i}$, the action predicted is $a_{pre} = a_{m}$, where $m = \arg\max_i f_i, i \in [0,c]$. Then the action alignment ratio is defined as:
																																																																																																																																																	
	% $$
	% \rho_r = \frac{1}{|S_r|}\sum_{(i, j) \in S_r} \mathbb{I}(a_{pre} = \hat{a}),a_{pre}\in z
	% $$


==> 05_RelatedWork.tex <==
% \begin{table*}[t]
%     \centering
%         \begin{tabular}{ p{4cm}||p{3.5cm}|p{2.6cm}|p{3cm}  }
%          \toprule
% %         \multicolumn{4}{c}{} \\
% %         \midrule
%          Method & QoI &Input Attribution&Special Treatment\\
%          \midrule
%          \citet{wang2015dueling} & Action & Saliency Map & N/A\\
%          \citet{Iyer2018TransparencyAE}& Action  &OC-1&   Template Matching\\
%          \citet{Greydanus2018VisualizingAU}& Action\&Distributional & OC-1   &Gaussian Blur\\
%          \citet{Puri2020ExplainYM} &Action\&Distributional & OC-1& $d(\xvec, \yvec) = \text{D}_\text{KL}(\xvec, \yvec)$ \\
%          \bottomrule
%         \end{tabular}
%     \caption{Attribution-based Explanation Tools}
%     \label{tab: existing work}
% \end{table*}

\section{Related Work}\label{sec: realted work}
% \noindent{\textbf{Attribution in Deep RL.}}
% We discuss several related work that have not been well-discussed in previous sections or the supplementary materials and how they are related to different QoI and input attribution methods. One line of work is Jacobian method~\cite{wang2015dueling}, which is equivalent to combining SM and Action QoI to identify important features. We then discuss two methods that both use Action QoI and OC-N but with different treatment to identify the baseline $b$ or the subset $\mathcal{D}$. Instead of perturbing the input with zeros, another approach is to perturb the input features with Gaussian blurs~\cite{Greydanus2018VisualizingAU}, which is equivalent to choosing the blurred pixels as a baseline $b$ and setting $N$ equal to the number of blurred pixels in OC-N. Template matching~\cite{10.5555/1643435} has also been used to identify a semantically meaningful subset of input features~\cite{Iyer2018TransparencyAE} , which is equivalent to setting $N$ equal to the number of pixels in the template in OC-N. Therefore, we consider Gaussian blurs and the template matching as two prepossessing techniques in applying OC-N to DQN models with image input instead of two different attribution methods. 

% \noindent\textbf{Action Reconstruction.} The concept of behavior-level explanation is largely motivated by the \textit{agreement} metric introduced by \citet{Annasamy2019TowardsBI} that reconstructs an action from the key-value in the proposed attention layer~\cite{Bahdanau2015NeuralMT}. Besides, It has shown with counterfactual analysis that reconstructing actions from an attribution map by human's judgement may not actually correspond to the agent's behavior~\cite{Atrey2020ExploratoryNE}, which also motivates the work of proposing concrete reconstruction rule, $\lambda$-BAR.

% \noindent\textbf{Attention.} On the other hand, using attentions belongs to another line of work which aims to build networks inherently explainable, which has been discussed both in general tasks~\cite{dong2017improving, Zhang2018InterpretableCN, Gao2020AnID} and deep RL~\cite{hayat2019inforl, Bera2020PODNetAN, Wang2020ExplanationOR}. 


% Most of proposed methods for interpreting RL models are based on post hoc saliency attribution to generate explanation of models. They explain a model after it has been trained. Prior work has employed Jacobian saliency methods to create explanations regarding agent behavior, highlighting which part is important to the agent when it makes the decision.\sm{Jacobian based saliency related work} \citet{Bogdanovic2015DeepAL} and \citet{zahavy2016graying} implemented saliency maps on different Atari games to generate pixel saliency then utilize it to explain the agent. \citet{yang2018learn} binarize the original Jacobian saliency and multiply it with original saliency and game frames.\sm{their first drawback}These Jacobian saliency based maps can not highlight specific environmental features that the agent is paying attention to, only generating explanation results that need further sematic interpretation of human. \sm{reasons why these methods do not perform well}For RL systems, the network weights are optimized for reducing the Bellman error and the effects of selected sequential actions can interact over long time periods, which contrasts with visual classification tasks where the deep models merely learn to map from images to labels. \sm{second drawback}They also do not provide a uniform evaluation metric to compare different attribution methods.

% \sm{related work about perturbation-based method}While pixel-level interventions are not guaranteed to produce meaningful changes in semantic concepts, saliency maps generated through perturbation from an object level result in more intuitive outcomes. \sm{how to do perturbation}Functionally, the perturbation can be achieved through various ways, including adding a gray mask\cite{Zeiler2014VisualizingAU}, blurring a small region with gaussian noise\cite{Greydanus2018VisualizingAU} or masking objects with the background color\cite{Iyer2018TransparencyAE}. \sm{how to compute QoI}As for the choice of QoI, \citet{Greydanus2018VisualizingAU} utilized squared difference between the value estimate of the original sequence and that of the perturbed one. \citet{Iyer2018TransparencyAE} 
% subtract perturbed Q value with the original one. They tend to produce saliency maps that are not specific to the action of interest, then \citet{Puri2020ExplainYM} introduce KL divergence and Harmonic mean to address this kind of specificity. \sm{some evaluation metrics for attribution methods of RL tasks}The evaluation of attribution under RL setting focuses on indicating which method is more interpretable for human to understand the agent's behavior. Some works include computing the similarity between action to be explained and action reconstructed by key-value in a proposed attention layer \cite{Annasamy2019TowardsBI}, human-experiments\cite{Iyer2018TransparencyAE,Puri2020ExplainYM}, and designing a loss to describe the gap between reconstructions of explanation and original important regions\cite{rupprecht2020finding}. \sm{our advantage}We proposed an uniform evaluation metric that is more semantic-preserving under RL setting.
 
% Another approach towards explainability in DRL is to train a network that is inherently explanable~\cite{mott2019interpretable, Shi2020SelfSupervisedDO}.  

% \citet{mott2019interpretable} add recurrent modules and attentions to help Q-Network to better learn the representations. They visualize and show that the input attribution of a DQN with attention structure has a better localization on the agent's goal.

% \pxm{Include in this section how these existing works are insufficient for our goals.}

% \paragraph*{Gradient-Based} Jacobian Saliency. Wang et al. (2015) extended gradient-based saliency maps to deep RL by computing the Jacobian of the output logits with respect to a stack of input images.

% \paragraph*{Perturbation-Based} Methods that compute the importance of an input feature by removing, altering, or masking the feature in a domain-aware manner and observing the change in output. Perturbation Saliency. Greydanus et al. (2017) generate saliency maps by perturbing the original input image using a Gaussian blur of the image and measure changes in policy from removing information from a region. Object Saliency. Iyer et al. (2018) use template matching, a common computer vision technique (Brunelli, 2009), to detect (template) objects within an input image and measure salience through changes in Q-values for masked and unmasked objects.

% \paragraph*{Attention-Based} Attention Saliency. Most recently, attention-based saliency mapping methods have been proposed to generate interpretable saliency maps (Mott et al., 2019; Nikulin et al., 2019).

% We are more interested in perturbation-based methods for black-box agents since it outperforms the gradient-based methods for the following reasons:
% \begin{enumerate}
%   \item Saliency map and integrated gradients use gradients of Q value wrt. input space to explain a decision of interest. But the pixels or regions highlighted by these methods are not always consistent with the semantic concepts of a game state. For instance, if we change the color of one feature and the saliency of the action we are interested in will change, but the agent only pays attention to the existence of this feature instead of the color density or feature shape. Thus these methods can not capture the core  of the features.
%   \item Smooth-Grad performs intervention $M$ to input space, adding gaussian noise to the input space and calculating the average of difference in logits produced by the original and modified images. Similarly, the intervention does not guarantee changes in game states. 
%   \item GradCAM uses class specific gradient information flowing into the last convolutional layer of the DQN for explaining a decision of interest. Here the class specific information refers to different kinds of action the agent possibly take. GradCAM can quantitively reflect the model's ability to identify "high-level" features to given output labels but the DQN model is not trained to learn the map from input space to action label, this method does not perform well.
%   \item Results produced by gradient-based methods under RL setting might lack physical meaning. When answering the question “What perturbation to the input increases a particular output?”, gradient methods can choose perturbations that lack physical meaning or which is not valid in a game process.
%   \item Also, gradient-based do not apply to scenarios with black-box access to the agent, and even with white-box access to model internals, they are not applicable when agents are not fully differentiable, such as the Pacman simulator we use, which input is binary matrix.
% \end{enumerate}


% % \carlee{Explain why prior work doesn't fully cover the differences between vision and RL explanations. Give some hints as to how to solve these issues (which we build on in the Methods section).}



% % \carlee{explain why Pacman is a good RL example/use case, and how our work generalizes beyond it. do we want to include MOVI too?}

% % Could show bad results in this section


==> 06_Discussion.tex <==
\section{Discussion}
\label{sec: discussion}
\paragraph{Why Gradient-Based Methods Perform Worse?} 


==> tikz_figure.tex <==
\begin{tikzpicture}
    \node (state) at (-1,-0.7) {$\mathbf{s}$};

    \node (n0_l0) at (0,0) {$h^0_0$};
    \node (n1_l0) at (0,-0.7) {$h^0_1$};
    \node (n2_l0) at (0, -1.4) {$h^0_2$};

    \node (n0_l1) at (1.2,0) {$h^1_0$};
    \node (n1_l1) at (1.2,-0.7) {$h^1_1$};
    \node (n2_l1) at (1.2, -1.4) {$h^1_2$};

    \node (n1_l2) at (2.4,-0.7) {$h^2_1$};
    
    \node (n_w) at (3.6,-0.7) {$n_w$};
    \node (n_q) at (4.8,-0.7) {$n_q$};

    \path (n0_l0) edge (n0_l1);
    \path (n0_l0) edge (n1_l1);
    \path (n0_l0) edge (n2_l1);
    
    \path (n1_l0) edge (n0_l1);
    \path (n1_l0) edge (n1_l1);
    \path (n1_l0) edge (n2_l1);
    
    \path (n2_l0) edge (n0_l1);
    \path (n2_l0) edge (n1_l1);
    \path (n2_l0) edge (n2_l1);
    
    \path (n0_l1) edge (n1_l2);
    \path (n1_l1) edge (n1_l2);
    \path (n2_l1) edge (n1_l2);
    
    \path (n1_l2) edge (n_w);
    \path (n_w) edge (n_q);

\end{tikzpicture} 
